"This Applies to the RealWorld": Student Perspectives on Integrating Ethics into a Computer Science Assignment

There is a growing movement in undergraduate computer science (CS) programs to embed ethics across CS classes rather than relying solely on standalone ethics courses. One strategy is creating assignments that encourage students to reflect on ethical issues inherent to the code they write. Building off prior work that has surveyed students after doing such assignments in class, we conducted focus groups with students who reviewed a new introductory ethics-based CS assignment. In this experience report, we present a case study describing our process of designing an ethics-based assignment and proposing the assignment to students for feedback. Participants in our focus groups not only shared feedback on the assignment, but also on the integration of ethics into coding assignments in general, revealing the benefits and challenges of this work from a student perspective. We also generated novel ethics-oriented assignment concepts alongside students. Deriving from tech controversies that participants felt most affected by, we created a bank of ideas as a starting point for further curriculum development.

==> table.tex <==

\begin{table*}[]
\begin{tabularx}{\textwidth}{XXXXXXXXX}
\textbf{P\#} & \textbf{Name}   & \textbf{Gender} & \textbf{Race}  & \textbf{Country} & \textbf{Institution}                 & \textbf{Department}                           & \textbf{Course}                                                     & \textbf{Position}                                 \\
1            & Neil Ernst      & Male            & White          & Canada           & The University of Victoria           & computer science                              & Ethical Issues in CS Research                                       & Assistant Professor                               \\
2            & Annuska Zolyomi & Female          & Latina         & USA              & The University of Washington Bothell & computing and software systems division       & Input and Interaction                                               & PhD Candidate  (now assistant teaching professor) \\
3            & Andrea Grover   & Female   & White          & USA              & University of Nebraska at Omaha      & Information Systems and Quantitative Analysis & IT Ethics                                                           & associate professor                               \\
4            & Morgan G. Ames  & Female          & White          & USA              & UC Berkeley                          & school of information                         & social issues of information and behind the data: humans and values & Assistant Adjunct Professor                       \\
5            & Victoria Dean   & Female   & White          & USA              & Carnegie Mellon university           & the robotics Institute                        & Ethics in Robotics                                                  & PhD Student                                       \\
6            & Robin Brewer    & Female  & Black          & USA              & university of Maryland, Michigan     & school of information                         & Introduction to Accessibility                                       & Assistant Professor                               \\
7            & Dan McQuillan   & Male            & White          & UK               & Goldsmiths, University of London     & department of computing                       & Ethical Computing                                                   & Lecturer                                          \\
8            &                 & Male            & White          & USA              & Rensselaer Polytechnic Institute     &                                               & Science, Technology, and Society                                    & Lecturer                                          \\
9            &                 & Male            & White          & USA              &                                      & Information Science                           &                                                                     & Instructor                                        \\
10           &                 & Male            & White          & Canada           &                                      &                                               & course on social media and digital life                             & Postdoc (now Instructor)                          \\
11           &                 & Female           & White          & USA              &                                      & iSchool                                       & Research Methods and Information Policy                             & Instructor                                        \\
12           &                 & Female           & White & UK               & Design School                        &                                               &                                                                     & Senior Lecturer                                  
\end{tabularx}
\end{table*}
